On the Structure, Covering, and Learning of Poisson Multinomial Distributions

An $(n,k)$-Poisson Multinomial Distribution (PMD) is the distribution of the sum of $n$ independent random vectors supported on the set ${\cal B}_k=\{e_1,\ldots,e_k\}$ of standard basis vectors in $\mathbb{R}^k$. We prove a structural characterization of these distributions, showing that, for all $\varepsilon >0$, any $(n, k)$-Poisson multinomial random vector is $\varepsilon$-close, in total variation distance, to the sum of a discretized multidimensional Gaussian and an independent $(\text{poly}(k/\varepsilon), k)$-Poisson multinomial random vector. Our structural characterization extends the multi-dimensional CLT of Valiant and Valiant, by simultaneously applying to all approximation requirements $\varepsilon$. In particular, it overcomes factors depending on $\log n$ and, importantly, the minimum eigenvalue of the PMD's covariance matrix from the distance to a multidimensional Gaussian random variable. We use our structural characterization to obtain an $\varepsilon$-cover, in total variation distance, of the set of all $(n, k)$-PMDs, significantly improving the cover size of Daskalakis and Papadimitriou, and obtaining the same qualitative dependence of the cover size on $n$ and $\varepsilon$ as the $k=2$ cover of Daskalakis and Papadimitriou. We further exploit this structure to show that $(n,k)$-PMDs can be learned to within $\varepsilon$ in total variation distance from $\tilde{O}_k(1/\varepsilon^2)$ samples, which is near-optimal in terms of dependence on $\varepsilon$ and independent of $n$. In particular, our result generalizes the single-dimensional result of Daskalakis, Diakonikolas, and Servedio for Poisson Binomials to arbitrary dimension.

==> abstract_text.tex <==
An (n,k)-Poisson Multinomial Distribution (PMD) is the distribution of the sum of n independent random vectors supported on the set B_k={e_1,...,e_k} of standard basis vectors in R^k. We prove a structural characterization of these distributions, showing that, for all epsilon > 0, any (n, k)-Poisson multinomial random vector is epsilon-close, in total variation distance, to the sum of a discretized multidimensional Gaussian and an independent (poly(k/epsilon), k)-Poisson multinomial random vector. Our structural characterization extends the multi-dimensional CLT of Valiant and Valiant, by simultaneously applying to all approximation requirements epsilon. In particular, it overcomes factors depending on log n and, importantly, the  minimum eigenvalue of the PMD's covariance matrix.

We use our structural characterization to obtain an epsilon-cover, in total variation distance, of the set of all (n,k)-PMDs, significantly improving the cover size of Daskalakis and Papadimitriou, and obtaining the same qualitative dependence of the cover size on n and epsilon as the k=2 cover of Daskalakis and Papadimitriou. We further exploit this structure to show that (n,k)-PMDs can be learned to within epsilon in total variation distance from ~O_k(1/epsilon^2) samples, which is near-optimal in terms of dependence on epsilon and independent of n.  In particular, our result generalizes the single-dimensional result of Daskalakis, Diakonikolas and Servedio for Poisson binomials to arbitrary dimension. Finally, as a corollary of our results on PMDs, we give a ~O_k(1/epsilon^2) sample algorithm for learning (n,k)-sums of independent integer random variables (SIIRVs), which is near-optimal for constant k.


==> rounding_backup.tex <==
\subsection{Rounding the Parameters}
\label{sec:rounding}

Fix some coordinate $x$, and select all $k$-CRVs where the parameter in coordinate $x$ is in the range $(0,c)$.
Partition this subset into $k-1$ sets, depending on which coordinate $y \neq x$ is the heaviest.
We apply a rounding procedure separately to each of these sets.
After this procedure, none of the parameters in coordinate $x$ will be in $(0,c)$.
We repeat this for all $k$ possible settings of $x$.
From the description below (and the restriction that $c \leq \frac{1}{2k}$), it will be clear that we will not ``undo'' any of our work and move probabilities back into $(0,c)$, so $O(k^2)$ applications of our rounding procedure will produce the result claimed in the theorem statement.

Recall that the goal of this rounding procedure will be to shift probability mass either to or from coordinate $x$ to coordinate $y$, such that no parameter in coordinate $x$ lies in the interval $(0,c)$, while simultaneously approximately preserving the mean vector of the distribution.
We are able to do this since coordinate $y$ is ``heavy'' and thus small additions will not affect the distribution in this coordinate much.

We fix some $x,y$ in order to describe and analyze the process more formally.
Define $\mathcal{I}^x_y = \{i\, |\, 0 < \r(i,x) < c \wedge y = \arg\max_j \r(i,j)\}$ (breaking ties lexicographically), and let $M^{\r_{I^x_y}}$ be the $(n,k)$-PMD induced by this set.
For the remainder of this section, without loss of generality, assume that the indices selected by $\mathcal{I}^x_y$ are $1$ through $|\mathcal{I}^x_y|$.

Select an arbitrary set $\mathcal{R} \subseteq \mathcal{I}^x_y$ such that $|\mathcal{R}| = \left\lfloor\frac{\sum_{i' \in I^x_y} \r_{I^x_y}(i',x)}{c}\right\rfloor$.
Intuitively, this set will be the CRVs for which we set the parameter $\r(\cdot,x)$ to be $c$, while $\mathcal{I}^x_y \setminus \mathcal{R}$ will have $\r(\cdot, x)$ set to $0$.
We can perform the following rounding scheme to $\r_{I^x_y}$ to obtain a new parameter matrix $\hat \r_{I^x_y}$:
$$
\hat \r_{I^x_y}(i,j) = 
\begin{cases}
  \r_{I^x_y}(i,j) &\mbox{if } j \not\in \{x,y\} \\ \vspace{1mm}
                c &\mbox{if } j = x \wedge i \in \mathcal{R} \\ 
                0 &\mbox{if } j = x \wedge i \not \in \mathcal{R} \\
 1 - \sum_{j' \neq y} \hat \r_{I^x_y}(i,j') &\mbox{if } j = y
\end{cases}
$$

%We first give the analysis for the total variation distance between the two PMDs. The analysis for this part doesn't depend at all on the set $\mathcal{R}$ but only on its size. We will take advantage of this flexibility in the choice of $\mathcal{R}$ later on to guarantee that the covariance matrix of the rounded PMD is coordinate-wise close to the original.

%\subsubsection{The rounded PMD is close in total variation to the original}
We define the process \textbf{Fork}, for sampling from a $k$-CRV $\r(i,\cdot)$ in $\mathcal{I}^x_y$:
\begin{itemize}
  \item Let $X_i$ be an indicator random variable, taking $1$ with probability $\frac{1}{k}$ and $0$ otherwise.
  \item If $X_i = 1$, then return $e_x$ with probability $k\r(i,x)$ and $e_y$ with probability $1 - k\r(i,x)$.
  \item If $X_i = 0$, then return $e_j$ with probability $0$ if $j = x$, $\frac{k}{k-1}(\r(i,x) + \r(i,y) - \frac1k)$ if $j = y$, and $\frac{k}{k-1}\r(i,j)$ otherwise.
\end{itemize}

The intuition behind this procedure is that we isolate the changes in our rounding procedure when $X_i = 1$, as when $X_i = 0$, the rounded and unrounded distributions are identical.
We note that \textbf{Fork} is well defined as long as $\r(i,x) \leq \frac{1}{k}$ and $\r(i,x) + \r(i,y) \geq \frac{1}{k}$.
The former is true since $c \leq \frac{1}{k}$, and the latter is true since $y$ was chosen to be the heaviest coordinate.
Additionally, by calculating the probability of any outcome, we can see that \textbf{Fork} is equivalent to the regular sampling process.
Define the (random) set $\bm{X} = \{i\, |\, X_i = 1\}$.
We will use $\bm{\th}$ to refer to a particular realization of this set.
We define \textbf{Fork} for sampling from $\hat \r(i,\cdot)$ in the same way, though we will denote the indicator random variables by $\hat X_i$ and $\bm{\hat X}$ instead.
Note that, if $c \leq \frac1k$, the process will still be well defined after rounding.
This is because $\hat \r(i,x) \leq c \leq \frac1k$, and $\hat \r(i,x) + \hat \r(i,y) = \r(i,x) + \r(i,y) \geq \frac1k$.
For the rest of this section, when we are drawing a sample from a CRV, we draw it via the process \textbf{Fork}.

The proof of Lemma \ref{lem:round} follows from the following lemmata: 
\begin{lemma}\label{lem:leaves}
  \begin{multline*}
    \Pr\left(\bm{\th} : \vphantom{ \sum_{i \in \bm{\th}}}\right.
     \left. \left|\sum_{i \in \bm{\th}} k\r_{I^x_y}(i,j) - E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,j)\Big]\right| 
    \leq \left(\frac{ck}{2} \log{\left(\frac{1}{ck}\right)}E \Big[\sum_{i \in \bm{X}}k \r_{I^x_y}(i,j)\Big]\right)^{1/2} \right. \\ 
  \wedge 
   \left. \left|\sum_{i \in \bm{\th}} k\hat \r_{I^x_y}(i,j) - E\Big[\sum_{i \in \bm{\hat X}}k\hat  \r_{I^x_y}(i,j)\Big]\right| 
  \leq \left(\frac{ck}{2} \log{\left(\frac{1}{ck}\right)}E \Big[\sum_{i \in \bm{\hat X}} k\hat \r_{I^x_y}(i,j)\Big]\right)^{1/2}
  \right) \\ \geq  1 - 4(ck)^{1/6}
  \end{multline*}
\end{lemma}

\begin{lemma}\label{lem:poisson}
  Suppose that, for some $\bm{\th}$, the following hold: 
$$\left|\sum_{i \in \bm{\th}} k\r_{I^x_y}(i,j) - E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,j)\Big]\right| 
    \leq \left(\frac{ck}{2} \log{\left(\frac{1}{ck}\right)}E \Big[\sum_{i \in \bm{X}}k \r_{I^x_y}(i,j)\Big]\right)^{1/2}$$

 $$ \left|\sum_{i \in \bm{\th}} k\hat \r_{I^x_y}(i,j) - E\Big[\sum_{i \in \bm{\hat X}}k\hat  \r_{I^x_y}(i,j)\Big]\right| 
  \leq \left(\frac{ck}{2} \log{\left(\frac{1}{ck}\right)}E \Big[\sum_{i \in \bm{\hat X}} k\hat \r_{I^x_y}(i,j)\Big]\right)^{1/2}$$
Then, letting $Z_i$ be the Bernoulli random variable with expectation $k \r_{I^x_y}(i,x)$ (and $\hat Z_i$ defined similarly with $ k\hat \r_{I^x_y}(i,x)$),
  $$\mathrm{d_{TV}}\left( \sum_{i \in \bm{\th}} Z_i,\sum_{i \in \bm{\th}} \hat Z_i  \right)
  < O\left(c^{1/2} k^{1/2} \log^{1/2}\left(\frac{1}{ck}\right)\right)$$
\end{lemma}

\begin{lemma}\label{lem:glue}
  For any $\mathcal{I}^x_y$,
  $$\dtv\left(M^{\r_{I^x_y}},M^{\hat\r_{I^x_y}}\right) < O\left(c^{1/2} k^{1/2} \log^{1/2}\left(\frac{1}{ck}\right)\right)$$
\end{lemma}
Since our final rounded $(n,k)$-PMD is generated after applying this rounding procedure $O(k^2)$ times, Lemma \ref{lem:round} follows from our construction and Lemma \ref{lem:glue} via the triangle inequality.

\begin{prevproof}{Lemma}{lem:leaves}
  Note that $\sum_{i \in \bm{X}} k\r_{I^x_y}(i,x) = \sum_{i \in I^x_y} \Om_i$, where 
  $$\Om_i = 
  \begin{cases}
    k\r_{I^x_y}(i,x) & \mbox{with probability } \frac1k \\
                   0 & \mbox{with probability } 1 - \frac1k
  \end{cases}
  $$
  We apply Lemma \ref{lem:cher} to the rescaled random variables $\Om_i' = \frac{1}{ck}\Om_i$, with $\g = \sqrt{\frac{\log{\frac1{ck}}}{2E[\sum_{i \in I^x_y} \Om_i']}}$, giving
  $$\Pr\left[\left|\sum_{i \in I^x_y} \Om_i' - E\Big[\sum_{i \in I^x_y} \Om_i'\Big]\right| \geq \left(\frac12 \log \left(\frac1{ck}\right)E\Big[\sum_{i \in I^x_y} \Om_i'\Big] \right)^{1/2}\right] \leq 2(ck)^{1/6}.$$
  Unscaling the variables gives
  \begin{multline*}
  \Pr\left[\left|\sum_{i \in \bm{X}} k\r_{I^x_y}(i,x) - E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,x) \Big]\right| \geq \left(\frac{ck}2 \log \left(\frac1{ck}\right) E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,x) \Big]\right)^{1/2}\right] \\ \leq 2(ck)^{1/6}.
  \end{multline*}

  Applying the same argument to $\hat \r_{I^x_y}$ gives 
  \begin{multline*}
  \Pr\left[\left|\sum_{i \in \bm{\hat X}} k\hat \r_{I^x_y}(i,x) - E\Big[\sum_{i \in \bm{\hat X}} k\hat \r_{I^x_y}(i,x) \Big]\right| \geq \left(\frac{ck}2 \log \left(\frac1{ck}\right) E\Big[\sum_{i \in \bm{\hat X}} k\hat \r_{I^x_y}(i,x) \Big]\right)^{1/2}\right]\\ \leq 2(ck)^{1/6}.
  \end{multline*}

  Since $\bm{X} \sim \bm{\hat X}$, by considering the joint probability space where $\bm{\th} = \bm{X} = \bm{\hat X}$ and applying a union bound, we get
  \begin{multline*}
    \Pr\left(\bm{\th} : \vphantom{ \sum_{i \in \bm{\th}}}\right.
     \left. \left|\sum_{i \in \bm{\th}} k\r_{I^x_y}(i,j) - E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,j)\Big]\right| 
    \leq \left(\frac{ck}{2} \log{\left(\frac{1}{ck}\right)}E \Big[\sum_{i \in \bm{X}}k \r_{I^x_y}(i,j)\Big]\right)^{1/2} \right. \\ 
  \wedge 
   \left. \left|\sum_{i \in \bm{\th}} k\hat \r_{I^x_y}(i,j) - E\Big[\sum_{i \in \bm{\hat X}}k\hat  \r_{I^x_y}(i,j)\Big]\right| 
  \leq \left(\frac{ck}{2} \log{\left(\frac{1}{ck}\right)}E \Big[\sum_{i \in \bm{\hat X}} k\hat \r_{I^x_y}(i,j)\Big]\right)^{1/2}
  \right)\\ \geq 1 - 4(ck)^{1/6}
  \end{multline*}
\end{prevproof}

\begin{prevproof}{Lemma}{lem:poisson}
  Fix some $\bm{\th} = \bm{X} = \bm{\hat X}$.
  Without loss of generality, assume $E \Big[\sum_{i \in \bm{X}}k \r_{I^x_y}(i,j)\Big] \geq E \Big[\sum_{i \in \bm{\hat X}}k\hat  \r_{I^x_y}(i,j)\Big]$.
  There are two cases:
  \begin{case}
    $ E \Big[\sum_{i \in \bm{X}}k \r_{I^x_y}(i,j)\Big] \leq (ck)^{3/4}$
  \end{case}
  From the first assumption in the lemma statement,
  \begin{align*}
    \sum_{i \in \bm{\th}} k\r_{I^x_y}(i,j) &\leq  E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,j)\Big]
    + \left(\frac{ck}{2} \log{\left(\frac{1}{ck}\right)}E \Big[\sum_{i \in \bm{X}}k \r_{I^x_y}(i,j)\Big]\right)^{1/2} \\
    &\leq (ck)^{3/4} + \frac{(ck)^{7/8}}{\sqrt{2}}\log^{1/2}{\left(\frac{1}{ck}\right)} \coloneqq g(c,k)
  \end{align*}
  Similarly, by the second assumption in the lemma statement and since \\
  $E \Big[\sum_{i \in \bm{X}}k \r_{I^x_y}(i,j)\Big] \geq E \Big[\sum_{i \in \bm{\hat X}}k\hat  \r_{I^x_y}(i,j)\Big],$
  we also have that
  $\sum_{i \in \bm{\th}} k\hat \r_{I^x_y}(i,j) \leq g(c,k)$.

  By Markov's inequality, $\Pr\Big[\sum_{i \in \bm{\th}} Z_i \geq 1\Big] \leq  \sum_{i \in \bm{\th}} k\r_{I^x_y}(i,j) \leq g(c,k)$,
  and similarly, $\Pr\Big[\sum_{i \in \bm{\th}} \hat Z_i \geq 1\Big] \leq g(c,k)$.
  This implies that $$\left| \Pr\Big[\sum_{i \in \bm{\th}} Z_i = 0\Big] - \Pr\Big[\sum_{i \in \bm{\th}} \hat Z_i = 0\Big] \right| \leq 2g(c,k),$$
  and thus by the coupling lemma,
  $$\dtv\left(\sum_{i \in \bm{\th}} Z_i,\sum_{i \in \bm{\th}} \hat Z_i\right) \leq 4g(c,k) = 4\left((ck)^{3/4} + \frac{(ck)^{7/8}}{\sqrt{2}}\log^{1/2}{\left(\frac{1}{ck}\right)} \right)$$
  

  \begin{case}
    $ E \Big[\sum_{i \in \bm{X}}k \r_{I^x_y}(i,j)\Big] \geq (ck)^{3/4}$
  \end{case}
  We use the following proposition, which is a combination of a classical result in Poisson approximation \cite{BarbourHJ92} and Lemma 3.10 in \cite{DaskalakisP07}.
  \begin{proposition}
    For any set of independent Bernoulli random variables $\{Z_i\}_i$ with expectations $E[Z_i] \leq ck$,
    $$\dtv\left(\sum_i Z_i,Poisson\Big(E\Big[\sum_i Z_i\Big]\Big)\right) \leq ck.$$
  \end{proposition}
  Applying this, we see
  $$\dtv\left(\sum_{i \in \bm{\th}} Z_i,Poisson\Big(E\Big[\sum_{i \in \bm{\th}} Z_i\Big]\Big)\right) \leq ck$$
  $$\dtv\left(\sum_{i \in \bm{\th}} \hat Z_i,Poisson\Big(E\Big[\sum_{i \in \bm{\th}} \hat Z_i\Big]\Big)\right) \leq ck$$
  We must now bound the distance between the two Poisson distributions.
  We use the following lemma from \cite{DaskalakisP08}:
  \begin{lemma}[Lemma B.2 in \cite{DaskalakisP08}]
    If $\l = \l_0 + D$ for some $D > 0, \l_0 > 0$,
    $$\dtv\left(Poisson(\l),Poisson(\l_0)\right) \leq D\sqrt{\frac{2}{\l_0}}.$$
  \end{lemma} 
  Applying this gives that 
  \begin{align*}
    &\dtv\left(Poisson\Big(E\Big[\sum_{i \in \bm{\th}} Z_i\Big]\Big),Poisson\Big(E\Big[\sum_{i \in \bm{\th}} \hat Z_i\Big]\Big)\right) \\
    &\leq
  \left|E\Big[\sum_{i \in \bm{\th}} Z_i\Big] - E\Big[\sum_{i \in \bm{\th}}\hat  Z_i\Big]\right| 
  \sqrt{\frac{2}{\min\left\{E\Big[\sum_{i \in \bm{\th}} Z_i\Big],E\Big[\sum_{i \in \bm{\th}}\hat Z_i\Big]\right\}}}
  \end{align*}

  To bound this, we need the following proposition, which we prove below:
  \begin{proposition}\label{prop:meanbound}
  $$\sqrt{\frac{2\left|\sum_{i \in \bm{\th}} k\r_{I^x_y}(i,x) - \sum_{i \in \bm{\th}} k\hat \r_{I^x_y}(i,x)\right|^2}
  {\min\left\{
    \sum_{i \in \bm{\th}} k \r_{I^x_y}(i,x),\sum_{i \in \bm{\th}} k\hat \r_{I^x_y}(i,x)
  \right\}}} \leq \sqrt{28ck\log\left(\frac{1}{ck}\right)}$$
  \end{proposition}

  Thus, using the triangle inequality and this proposition, for sufficiently small $c$, we get
  $$\dtv\left(\sum_{i \in \bm{\th}} Z_i,\sum_{i \in \bm{\th}} \hat Z_i\right) \leq 2ck + \sqrt{28ck\log\left(\frac{1}{ck}\right)} = O\left(c^{1/2}k^{1/2}\log^{1/2}\left(\frac1{ck}\right)\right).$$

  By comparing Cases 1 and 2, we see that the desired bound holds in both cases.

  \begin{prevproof}{Proposition}{prop:meanbound}
    By the definition of our rounding procedure, we observe that 
    $$\left|E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,x) \Big] - E\Big[\sum_{i \in \bm{\hat X}} k\hat \r_{I^x_y}(i,x) \Big]\right| \leq c$$
    By the assumptions of Lemma \ref{lem:poisson} and the assumption that $E \Big[\sum_{i \in \bm{X}}k \r_{I^x_y}(i,j)\Big] \geq E \Big[\sum_{i \in \bm{\hat X}}k\hat  \r_{I^x_y}(i,j)\Big]$,
    \begin{align*}
      \left|\sum_{i \in \bm{\th}} k\r_{I^x_y}(i,x) - \sum_{i \in \bm{\th}} k\hat \r_{I^x_y}(i,x)\right|  
      &\leq \left|E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,x) \Big] - E\Big[\sum_{i \in \bm{\hat X}} k\hat \r_{I^x_y}(i,x) \Big]\right| \\
      &+ \left(2ck\log\left(\frac{1}{ck}\right) E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,x) \Big]\right)^{1/2} \\
      &\leq c + \left(2ck\log\left(\frac{1}{ck}\right) E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,x) \Big]\right)^{1/2},
    \end{align*}
    and thus,
    \begin{align} 
      &\left|\sum_{i \in \bm{\th}} k\r_{I^x_y}(i,x) - \sum_{i \in \bm{\th}} k\hat \r_{I^x_y}(i,x)\right|^2 \nonumber \\
      &\leq c^2 + 2ck\log\left(\frac{1}{ck}\right) E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,x) \Big] + \left(8c^3k\log\left(\frac{1}{ck}\right) E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,x) \Big]\right)^{1/2} \label{eq:num}
    \end{align}
    From the assumption that $E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,x) \Big] \geq (ck)^{3/4}$, for sufficiently small $c$,
    \begin{align*}
      E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,x) \Big] &\geq (ck)^{3/8}\left(E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,x) \Big]\right)^{1/2} \\
                                                       &\geq \left(2ck \log{\left(\frac{1}{ck}\right)}E \Big[\sum_{i \in \bm{X}}k \r_{I^x_y}(i,j)\Big]\right)^{1/2}
    \end{align*}

    Combining this with the first assumption of Lemma \ref{lem:poisson}, 
    \begin{align*}
      \sum_{i \in \bm{\th}} k\r_{I^x_y}(i,x) &\geq E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,x) \Big] - \left(\frac{ck}{2} \log{\left(\frac{1}{ck}\right)}E \Big[\sum_{i \in \bm{X}}k \r_{I^x_y}(i,j)\Big]\right)^{1/2} \\
  &\geq \frac12 E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,x) \Big] 
  \end{align*}
  Similarly, since 
  $E \Big[\sum_{i \in \bm{\hat X}}k\hat  \r_{I^x_y}(i,j)\Big] \geq E \Big[\sum_{i \in \bm{X}}k \r_{I^x_y}(i,j)\Big] - c \geq (ck)^{3/4} - c$, for $c$ sufficiently small,
  $$\sum_{i \in \bm{\th}} k\hat \r_{I^x_y}(i,x) \geq \frac12 E\Big[\sum_{i \in \bm{X}} k\hat \r_{I^x_y}(i,x) \Big]$$

  It follows that
  \begin{align}
    &\min\left\{\sum_{i \in \bm{\th}} k \r_{I^x_y}(i,x),\sum_{i \in \bm{\th}} k\hat \r_{I^x_y}(i,x) \right\}\nonumber  \\
    &\geq \frac12 \min\left\{E\Big[\sum_{i \in \bm{X}} k \r_{I^x_y}(i,x)\Big],E\Big[\sum_{i \in \bm{\hat X}} k\hat \r_{I^x_y}(i,x)\Big] \right\}\nonumber  \\
    &= \frac12 E\Big[\sum_{i \in \bm{\hat X}} k\hat \r_{I^x_y}(i,x)\Big] \nonumber \\
    &\geq \frac12 \left(E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,x)\Big] - c\right) \nonumber \\
    &\geq \frac14 E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,x)\Big] \label{eq:den}
  \end{align}
  where the last equality follows for $c$ sufficiently small because $E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,x)\Big] \geq (ck)^{3/4}$.

  From (\ref{eq:num}) and (\ref{eq:den}), for $c$ sufficiently small,
  $$\frac{2\left|\sum_{i \in \bm{\th}} k\r_{I^x_y}(i,x) - \sum_{i \in \bm{\th}} k\hat \r_{I^x_y}(i,x)\right|^2}
  {\min\left\{
    \sum_{i \in \bm{\th}} k \r_{I^x_y}(i,x),\sum_{i \in \bm{\th}} k\hat \r_{I^x_y}(i,x)
  \right\}} \leq 28ck\log\left(\frac{1}{ck}\right),$$
  from which the proposition statement follows.
  \end{prevproof}
\end{prevproof}

\begin{prevproof}{Lemma}{lem:glue}
  Throughout this proof, we will couple the two sampling processes such that $\bm{\th} \coloneqq\bm{X} = \bm{\hat X} $, which is possible since $\bm{X} \sim \bm{\hat X}$.
  Let $\phi$ be the random event that $\bm{\th}$ satisfies the following conditions:
  \begin{align*}
    & \left. \left|\sum_{i \in \bm{\th}} k\r_{I^x_y}(i,j) - E\Big[\sum_{i \in \bm{X}} k\r_{I^x_y}(i,j)\Big]\right| 
    \leq \left(\frac{ck}{2} \log{\left(\frac{1}{ck}\right)}E \Big[\sum_{i \in \bm{X}}k \r_{I^x_y}(i,j)\Big]\right)^{1/2} \right. \\ 
  & \left|\sum_{i \in \bm{\th}} k\hat \r_{I^x_y}(i,j) - E\Big[\sum_{i \in \bm{\hat X}}k\hat  \r_{I^x_y}(i,j)\Big]\right| 
  \leq \left(\frac{ck}{2} \log{\left(\frac{1}{ck}\right)}E \Big[\sum_{i \in \bm{\hat X}} k\hat \r_{I^x_y}(i,j)\Big]\right)^{1/2}
  \end{align*}
 
  Suppose that $\phi$ occurs, and fix a $\bm{\th}$ in this probability space.
  We start by showing that for such a $\bm{\th}$, 
  $$\mathrm{d_{TV}}\left(M^{\r_{I^x_y}},M^{\hat\r_{I^x_y}}\, \middle|\, \bm{X} = \bm{\hat X} = \bm{\th}\right) < O\left(c^{1/2} k^{1/2} \log^{1/2}\left(\frac{1}{ck}\right)\right)$$
  Let $M^{\r_{I^x_y}^{\bm{\th}}}$ and $M^{\r_{I^x_y}^{\bm{\bar\th}}}$ be the $(n,k)$-PMDs induced by the $k$-CRVs in $M^{\r_{I^x_y}}$ with indices in $\bm{\th}$ and not in $\bm{\th}$, respectively.
  Define $M^{\hat \r_{I^x_y}^{\bm{\th}}}$ and $M^{\hat \r_{I^x_y}^{\bm{\bar\th}}}$ similarly.
  We can see
  \begin{align*}
  \mathrm{d_{TV}}\left(M^{\r_{I^x_y}},M^{\hat\r_{I^x_y}}\, \middle|\, \bm{X} = \bm{\hat X} = \bm{\th}\right)
  &= \mathrm{d_{TV}}\left(M^{\r_{I^x_y}^{\bm{\th}}} + M^{\r_{I^x_y}^{\bm{\bar\th}}},
                         M^{\hat \r_{I^x_y}^{\bm{\th}}} + M^{\hat \r_{I^x_y}^{\bm{\bar\th}}}
  \middle|\, \bm{X} = \bm{\hat X} = \bm{\th}\right) \\
  &\leq \mathrm{d_{TV}}\left(M^{\r_{I^x_y}^{\bm{\th}}}, M^{\hat \r_{I^x_y}^{\bm{\th}}}  \middle|\, \bm{X} = \bm{\hat X} = \bm{\th}\right) \\
  &+ \mathrm{d_{TV}}\left(M^{\r_{I^x_y}^{\bm{\bar \th}}}, M^{\hat \r_{I^x_y}^{\bm{\bar \th}}}  \middle|\, \bm{X} = \bm{\hat X} = \bm{\th}\right) \\
  &\leq \mathrm{d_{TV}}\left(M^{\r_{I^x_y}^{\bm{\th}}}, M^{\hat \r_{I^x_y}^{\bm{\th}}}  \middle|\, \bm{X} = \bm{\hat X} = \bm{\th}\right) \\
  &= \mathrm{d_{TV}}\left(\sum_{i \in \bm{\th}} Z_i,\sum_{i \in \bm{\th}} \hat Z_i  \middle|\, \bm{X} = \bm{\hat X} = \bm{\th}\right) \\
  &\leq O\left(c^{1/2}k^{1/2}\log^{1/2}\left(\frac1{ck}\right)\right)
  \end{align*}
  The first inequality is the triangle inequality,
  the second inequality is because the distributions for $k$-CRVs in $\bm{\bar \th}$ are identical (since we do not change them in our rounding),
  and the third inequality is Lemma \ref{lem:poisson}.

  By the law of total probability for total variation distance,
  \begin{align*}
  \mathrm{d_{TV}}\left(M^{\r_{I^x_y}},M^{\hat\r_{I^x_y}}\right) 
  &= \Pr(\phi)\mathrm{d_{TV}}\left(M^{\r_{I^x_y}},M^{\hat\r_{I^x_y}} \middle| \phi \right)
  + \Pr(\bar \phi)\mathrm{d_{TV}}\left(M^{\r_{I^x_y}},M^{\hat\r_{I^x_y}} \middle| \bar \phi \right) \\
  &\leq \left(1 - 4(ck)^{1/6}\right) \cdot O\left(c^{1/2}k^{1/2}\log^{1/2}\left(\frac1{ck}\right)\right) + 4(ck)^{1/6} \cdot 1 \\
  &= O\left(c^{1/2}k^{1/2}\log^{1/2}\left(\frac1{ck}\right)\right)
  \end{align*}
  where the inequality is obtained by applying Lemma \ref{lem:leaves} and the bound shown above pointwise for $\bm{\th}$ which satisfy $\phi$.

\end{prevproof}

%\subsubsection{Bounding the mean and covariance}

%We now show that for every pair $x,y$ there exists a set $\mathcal{R} \subseteq \mathcal{I}^x_y$ with $|\mathcal{R}| = \left\lfloor\frac{\sum_{i \in I^x_y} \r_{I^x_y}(i,x)}{c}\right\rfloor$ such that the mean and covariance of the rounded PMD are coordinate-wise close to the original. In particular, we will show that for all pairs of coordinates $a,b$:
%$$| \mu^{\r}_a - \mu^{\hat{\r}}_a | \le c$$
%$$| \Sigma^{\r}_{a,b} - \Sigma^{\hat{\r}}_{a,b} | \le ( | \Sigma^{\r}_{a,b} | + 8) k c$$
%The theorem will follow as we perform the rounding process at most $k^2$ times. 


%Since both the mean and covariance is additive, we can focus only on the set $I^x_y$.

%The fact that the mean is close follows directly from the size of $\mathcal{R}$. During the rounding process for $x,y$ only coordinates $x$ and $y$ of the mean are affected. The size of $\mathcal{R}$ is such that $0 \le \mu^{\r}_x - \mu^{\hat{\r}}_x  \le c$, and since $\mu^{\r}_y = | I^x_y | - \sum_{j \neq y} \mu^{\r}_j$ it also holds that $0 \ge \mu^{\r}_y - \mu^{\hat{\r}}_y  \ge -c$.

%For the covariance matrix, we have that $\Sigma^{\hat{\r}}_{a,b} = -\sum_i \hat{\r}(i,a) \hat{\r}(i,b)$ for $a \neq b$ and $\Sigma^{\hat{\r}}_{a,a} = \sum_i \hat{\r}(i,a) (1-\hat{\r}(i,a))$.  
%This implies that $\Sigma^{\hat{\r}}_{a,b}  = \Sigma^{{\r}}_{a,b}$, if both $a,b \in [k] \setminus \{x,y\}$ since those elements are not affected by the rounding.
%Moreover, the bound holds for $\Sigma^{\hat{\r}}_{x,x}$ since
%$$\Sigma^{\hat{\r}}_{x,x} = \sum_i \hat{\r}(i,x) (1-\hat{\r}(i,x)) \ge (1-c) \sum_i \hat{\r}(i,x) \ge (1-c) \sum_i {\r}(i,x) - c \ge (1-c) |\Sigma^{{\r}}_{x,x}| - c$$
%and
%$$\Sigma^{{\r}}_{x,x} = \sum_i {\r}(i,x) (1-{\r}(i,x)) \ge (1-c) \sum_i {\r}(i,x) \ge
%(1-c) \sum_i \hat{\r}(i,x) = \Sigma^{\hat{\r}}_{x,x}$$


%To bound the rest of the entries, we will make use of the following lemma which gives us a way to pick the rounding scheme so that the rounded coordinates are close to the original ones.

%\begin{lemma}
%\label{lem:pickingR}
%There exists a set $\mathcal{R}$ with $|\mathcal{R}| = \left\lfloor\frac{\sum_{i \in I^x_y} \r (i,x)}{c}\right\rfloor$, such that for the induced rounding scheme it holds for all $j$:
%\begin{itemize}
%\item $|\sum_i {\r}(i,j) {\r}(i,x) - \sum_i {\r}(i,j) \hat{\r}(i,x)| \le 4 k c$ and 
%\item $|\sum_i {\r}(i,j) {\r}(i,y) - \sum_i {\r}(i,j) \hat{\r}(i,y)| \le 4 k c$.
%\end{itemize}
%\end{lemma}

%\begin{proof}
%We have that $\hat{\r}(i,x) = {\r}(i,x) + \delta_i$ and $\hat{\r}(i,y) = {\r}(i,y) - \delta_i$
%where $\delta_i = c - {\r}(i,x)$ if rounding up or $\delta_i = 0 - {\r}(i,x)$ if rounding down.

%We let $P$ be a $n \times (2k+1)$ matrix with entries: 
%$$
%P_{i,j} = 
%\begin{cases}
%  \r(i,j) &\mbox{if } 1 \le j \le k \\ \vspace{1mm}
% -\r(i,j) &\mbox{if } k+1 \le j \le 2 k \\ 
%                1 &\mbox{if } j = 2 k + 1
%\end{cases}
%$$
%We will show that there exists a vector $\delta$ such that $| \delta^T \cdot P   |_{\infty} \le 2 k c$. This can be thought of as the Minkowski sum of the sets $\{-\r(i,x) P_i, (c - \r(i,x)) P_i\}$ where $P_i$ is the $i$-th row of the matrix $P$. We note that the vector $0$ lies in the convex hull of the above Minkowski sum. By the Starr's Corollary to the Shapley-Folkman theorem, and since the radius in terms of eucledian distance of each set is at most $\frac 3 2 c$, there is a point in the Minkowski sum that is within eucledian distance at most $\frac 3 2 c \sqrt{2 k+1} \le 2 k c$ for $k \ge 2$. Thus, $| \delta^T \cdot P   |_2 \le 2 k c$ which implies that $| \delta^T \cdot P   |_{\infty} \le 2 k c$.

%Although, this gives us the bound we want, it might not satisfy the size constraint on $\mathcal{R}$. We have however that $| \sum_i \delta_i | \le 2 k c$, which means that $| c |\mathcal{R}| - \sum_i \r(i,x)| \le 2 k c$. This means that we can satisfy the constraint $|\mathcal{R}| = \left\lfloor\frac{\sum_{i \in I^x_y} \r (i,x)}{c}\right\rfloor$ by adding or removing at most $2 k$ coordinates in the set $\mathcal{R}$. This affects the rest of the linear constraints by at most $2 k c$, so we can construct a $\delta$ so that $| \delta^T \cdot P   |_{\infty} \le 4 k c$.
%\end{proof}

%We now make use of the Lemma \ref{lem:pickingR}, to bound the remaining entries in the covariance matrix.

%For the entries $\Sigma^{\hat{\r}}_{x,a}$ or $\Sigma^{\hat{\r}}_{y,a}$, with $a \in [k] \setminus  \{x,y\}$, the lemma gives us the result directly. 

%Finally, for the entries $\Sigma^{\hat{\r}}_{x,y}$ and $\Sigma^{\hat{\r}}_{y,y}$, we note that since ${\r}(i,y) \ge \frac 1 k$, we have that $\hat{\r}(i,y) \ge {\r}(i,y) - c \ge (1-c k) {\r}(i,y)$ and similarly $\hat{\r}(i,y) \le (1+c k) {\r}(i,y)$. So, for $\Sigma^{\hat{\r}}_{y,y}$, we have that:
%$$\Sigma^{\hat{\r}}_{y,y} = \sum_i \hat{\r}(i,y) (1-\hat{\r}(i,y)) \in \left[ 1-ck , 1+ck \right] \cdot \sum_i {\r}(i,y) (1-\hat{\r}(i,y)) $$
%But since $| \sum_i {\r}(i,y) (1-\hat{\r}(i,y)) - \sum_i {\r}(i,y) (1-{\r}(i,y))| \le 4 c k$, we have that $|\Sigma^{\hat{\r}}_{y,y} - \Sigma^{{\r}}_{y,y}| \le |\Sigma^{{\r}}_{y,y}| c k + (1+ck) 4 ck \le ( |\Sigma^{{\r}}_{y,y}| + 8) ck$.

%Similarly, for $\Sigma^{\hat{\r}}_{y,x}$, we have that:
%$$\Sigma^{\hat{\r}}_{y,x} = - \sum_i \hat{\r}(i,y) \hat{\r}(i,x) \in \left[ 1-ck , 1+ck \right] \cdot \sum_i {\r}(i,y) \hat{\r}(i,x) $$
%which also gives that $|\Sigma^{\hat{\r}}_{x,y} - \Sigma^{{\r}}_{x,y}| \le ( |\Sigma^{{\r}}_{x,y}| + 8) ck$. 


